Measuring Geographic Performance Disparities of Offensive Language Classifiers

Text classifiers are applied at scale in the form of one-size-fits-all solutions. Nevertheless, many studies show that classifiers are biased regarding different languages and dialects. When measuring and discovering these biases, some gaps present themselves and should be addressed. First, ``Does language, dialect, and topical content vary across geographical regions?'' and secondly ``If there are differences across the regions, do they impact model performance?''. We introduce a novel dataset called GeoOLID with more than 14 thousand examples across 15 geographically and demographically diverse cities to address these questions. We perform a comprehensive analysis of geographical-related content and their impact on performance disparities of offensive language detection models. Overall, we find that current models do not generalize across locations. Likewise, we show that while offensive language models produce false positives on African American English, model performance is not correlated with each city's minority population proportions. Warning: This paper contains offensive language.

==> Sections/Conclusion.tex <==
%We provide a comprehensive analysis that highlights the strengths of current methods for model selection, while providing real-world recommendations for different model selection scenarios (e.g., when a auxiliary out-of-domain dataset is available). Unsupervised domain adaptation model selection metrics can facilitate a wide range of applications in the NLP community. For instance, if we can effectively rank the performance of models to novel groups of data, then we can potentially improve the fairness of deployed models and even begin to understand potential language characteristics that certain models perform poorly on because of inductive biases by evaluating models at scale.

We provide a comprehensive analysis of performance disparities of offensive language detection models. Furthermore, we introduce a novel dataset that provides more than 14 thousand examples for further analysis of geographical differences in model performance. The study points to the importance of community-driven NLP, where the impact and performance of NLP models are analyzed for specific communities, or even micro communities within a city. Moreover, finding communities that models perform poorly on can also provide unique testbeds as ``hard test cases'' similar to recent work on adversarial examples~\cite{zhang2019generating}.

==> Sections/DataCollection.tex <==
\section{Data}

%To test our methods on deciding which classifier to deploy in different situations, we leverage 3 labeled datasets as well as a dataset collected using the Twitter API which we call the Geo Offensive Language Identification. A brief description for each dataset is described below and an explanation on how the datasets were transformed to fit our needs in detecting offensive language on Twitter.

In this section, we describe the two major datasets used in our experiments: the Offensive Language Identification Dataset~(OLID)~\cite{zampieri2019predicting} and our newly constructed Geographical Diverse Offensive Language Identification Dataset (GeoOLID). A complete summary of the datasets can be found in Table~\ref{tab:datasets}. The OLID datasets was split into 5 random 70/10/20 training, validation, and testing splits, respectively. The GeoOLID dataset is only used for testing.

\begin{comment}
\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{mde.pdf}
    \caption{MDE}
    \label{fig:my_label}
\end{figure}
\end{comment}

\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllll} \toprule
\textbf{} & \textbf{Non Offensive} & \textbf{Offensive} & \textbf{Total} & \textbf{MDE}  \\ \midrule
\textbf{OLID} & 9,460 & 4,640 & 14,100 & .014 \\ \midrule \midrule
& \multicolumn{4}{c}{\textbf{GeoOLID Dataset}} \\ \midrule
& \textbf{Non Offensive} & \textbf{Offensive} & \textbf{Total}  & \textbf{MDE} \\ \midrule
\textbf{Unlabeled Data} & --- & ---  & 34,724 & --- \\
\textbf{All Cities (labeled)} & 9,259 & 4,831 & 14,090  \\  \midrule
\textbf{City Name} & \textbf{Non Offensive} & \textbf{Offensive} & \textbf{Total} & \textbf{MDE} \\ \midrule
Baltimore, MD & 630 & 277 & 907 & .054\\
Chicago, IL & 676 & 326 & 1002 & .052 \\
Columbus, OH & 616 & 301 & 917 & .054 \\
Detroit, MI & 549 & 367 & 916 &  .053 \\
El Paso, TX & 502 & 404 & 906 & .055 \\
Houston, TX & 635 & 297 & 932 & .054 \\
Indianapolis, IN & 600 & 307 & 907 & .055 \\
Los Angeles, CA & 660 & 298 & 958 & .053 \\
Memphis, TN & 564 & 368 & 932 & .054  \\
Miami, FL & 726 & 216 & 942 & .054 \\
New Orleans, LA & 607 & 325 & 932 & .054 \\
New York, NY & 717 & 265 & 982 & .053 \\
Philadelphia, PA & 629 & 337 & 966 & .054 \\
Phoenix, AZ & 577 & 355 & 932 & .054 \\
San Antonio, TX & 572 & 387 & 959 & .053 \\ \bottomrule
\end{tabular}%
}
\caption{Dataset Statistics.\vspace{-2em}}
\label{tab:datasets}
\end{table}


\vspace{1mm} \noindent \textbf{OLID.}
The OLID dataset introduced by \citet{zampieri2019predicting} contains 14,100 tweets labeled to identify different levels of offensiveness including, but not limited to, Not Offensive, Offensive, Targeted Offense, and Not Targeted Offense. Furthermore, Targeted Offenses are sub-categorized as targeting an individual, group, or other. For this study, we use the first level: Not Offensive (9,460 Total)and Offensive~(4,640 Total). 


\vspace{1mm} \noindent \textbf{GeoOLID.}
In addition to the OLID dataset, we introduce a new offensive language dataset using tweets collected since the start of the COVID-19 pandemic. \citet{qazi_geocov19_sigspatial} and \citet{lamsal2021design} originally collected more than 524 million multilingual tweets across 218 countries and 47,000 cities between the dates of February 1, 2020 and May 1, 2020. Given the large amount of politically divisive discourse, racist remarks, and social impact of COVID-19, GeoOLID provides a unique testbed to understand geographic model variation.

\vspace{1mm} \noindent \textbf{Filtering:} To filter down the 524 million tweets into a manageable set for this study, we first selected English Language tweets only. English Language tweets are then filtered by city, only keeping geocoded tweets with a coordinate point tied to a city of origination. We then subset all cities, removing any tweet not posted from a small group of 15 manually chosen cities that differ geographically and demographically. %This provides us with a substantial amount of data to detect hate speech during the COVID-19 pandemic. 

With the goal of identifying offensive language, we wanted to guarantee there was a mixture of normal and offensive tweets present in each city. Our last filter included a keyword filter using the badword lexicon~\cite{von2009offensive}, hatebase lexicon~\cite{davidson2017automated}, offensive phrases used for the original OLID dataset~\cite{zampieri2019predicting} (you are, she is, he is, conservatives, liberals, MAGA, and antifa), and additional COVID-specific phrases that we deem relevant for potential discrimination against a race (chinese, china, asia, asian, wuhan). Along with the aforementioned filters we appended on a sub sample of tweet data for each city and drop any replicated tweets. The final counts of each city can be found in Table \ref{tab:datasets}.

%How were the cities chosen 
\vspace{1mm} \noindent \textbf{Cities:} To measure the performance difference across varying geolocations, we decided on 15 cities based on multiple facets, data availability, annotation time, geographical diversity, and demographic diversity.
When selecting the 15 cities we strategically selected locations in the United States that different dialects could be present, as well as the topic distribution.
For example, cities like Baltimore, Memphis, New Orleans, and Detroit were chosen due to the high proportion of African Americans populations while, Indianapolis and Columbus had high proportions of White Non-Hispanic residents. El Paso, San Antonio and Phoenix have a close proximity to the Mexico boarder and higher percentage of Latino and Hispanic residents, which is very different from Columbus and Chicago. In addition we selected cities where we knew residents could use very distinct accents and phonics like New York and New Orleans. By selecting the 15 cities in Table \ref{tab:datasets}, we created a diverse dataset with multiple ethnicities, language styles, and topical differences.  


%How they were annotated
\vspace{1mm} \noindent \textbf{Annotation:} In order to provide accurate labels for this study, samples of 500 tweets were assigned to 3 different graduate students to be labeled as offensive language using the logic provided by ~\newcite{zampieri2019predicting}. A total of 20 students were recruited and given a stipend of \$100 for their time and effort. Several meetings were set up before labeling started to answer questions and address implications. The definition of an Offensive tweet was provided as \textit{Tweets containing any form of non-acceptable language (profanity) or a targeted offense, which can be veiled or direct. This includes insults, threats, and posts containing profane language or swear words.} 

\begin{table}[t]
\centering
\resizebox{0.7\linewidth}{!}{%
\begin{tabular}{lrr}
\toprule
                 & \textbf{F1}   & \textbf{Acc.} \\ \midrule
%\multicolumn{3}{c}{\textbf{Random Baselines}} \\ \midrule
\textbf{Stratified}               & .059 & .056     \\
\textbf{Uniform}             & .062 & .062     \\
\textbf{Prior}                 & .008 & .068     \\ \midrule 
%\multicolumn{3}{c}{\textbf{Content vs. Stylistic Features}} \\ \midrule
\textbf{BoW}                & .430 & .380     \\
\textbf{POS}              & .410 & .356     \\
\textbf{Dialect}               & .374 & .366     \\ \midrule 
%\multicolumn{3}{c}{\textbf{Combinations}} \\ \midrule
\textbf{POS +   Dialect}     & .419 & .357     \\
\textbf{BoW +   Dialect}      & \textbf{.436} & \textbf{.381}     \\
\textbf{BoW + POS +   Dialect}    &   .431 & .370         \\ \bottomrule
\end{tabular}%
}
\caption{Location prediction. Accuracy, Macro Precision, Macro Recall, and Macro F1.\vspace{-2em}}
\label{tab:city_pred}
\end{table}

Following general annotation recommendations for NLP~\cite{pustejovsky2012natural}, the annotation process was completed in three stages. First, the graduate students annotated the tweets, providing us with 3 separate independent labels of each tweet. We then calculated the agreement between annotators, resulting in a Fleiss Kappa of 0.47. This agreement score was not sufficient enough for us to feel comfortable running experiments on. Second, we (the authors) of the paper manually---and independently---adjudicated the annotation of each user, correcting miss-annotated tweets that were not agreed on by all three annotators. Common issues found during the process were labels of ``Not Offensive'' for tweets with ad-hoc mentions of the ``Wuhan Virus'' and offensive content found in the hashtag.  Third, one of the authors went through the tweets once again correcting any final disagreements among the authors adjudications, forming the final dataset described in Table~\ref{tab:datasets}. After collecting and adjudicating the responses, the total number of Offensive tweets were 4,831 compared to 9,259 Not Offensive and the final agreement score increased to 0.83. Finally, we report Minimum Detectable Effect (MDE)~\cite{card2020little} for Accuracy in Table~\ref{tab:datasets}. Specifically, use the Binomial Power Test, which assumes that samples are unpaired, i.e., the new model and baseline evaluation samples are drawn from the same data distribution but are not necessarily the same samples. The MDE numbers assume an accuracy of .75, which results in a significant difference between two models being around .05. We plot more potential MDE scores for different baseline numbers in the Appendix.


\vspace{1mm}
\noindent \textbf{Unlabeled GeoOLID Data.} We also make use of unlabeled and unfiltered data that GeoOLID was sampled from. The basic stats of this dataset are available in Table~\ref{tab:datasets} in the row titled ``Unlabeled Data''. The data is the same as the labeled GeoOLID, except it was not labeled because of resource constraints. 




%\vspace{1mm} \noindent \textbf{Geographical Disparities in Language: } 
%For our dataset to be novel and contribute to the current research, our dataset needs to capture disparities in language across the different location. We use 3 different techniques to show case that there exists a difference in language across the cities. 

 































\begin{comment}

\vspace{1mm} \noindent \textbf{FOUNTA.}
\citet{founta2018large} published a large-scale crowdsourced abusive tweet dataset with 60K total tweets. They identify abusive behaviors on Twitter with the categories None, Spam, Abusive, and Hateful, resulting in 11\% labeled as `Abusive,' 7.5\% as `Hateful,' 22.5\% as `Spam,' and 59\% as `None.' We then followed the work of \citet{park2018reducing} and transform the dataset into a binary task by combining Spam and None classes into a ``Not Offensive'' class (37,775 Total) and the Hateful/Abusive classes into an ``Offensive'' class (22240 Total).



\vspace{1mm} \noindent \textbf{WASEEM.}
The tweets collected by \newcite{waseem2016hateful} and used in \newcite{waseem2016you} were annotated by experts for three different categories: `Sexist', `Racist', or `Neither'. Like the FOUNTA dataset, we combine the Sexist and Racist tweets into an Offensive category (2856 Total), and the Neither tweets form the Not Offensive class~(7951~Total).
\end{comment}

==> Sections/Discussion.tex <==
In this section, we describe the general implications of this study to NLP practitioners, both in industry and academia. 

\vspace{1mm} \noindent \textbf{Impact on NLP Practitioners.} In industry, a budget it typically given to model builders to build and maintain a solution for NLP problems. Resources are not unlimited and definitely are not cheap. By using our proposed method, the time, effort, and costs of building these models will not be wasted. With saving the models for future deployment and reusability, NLP practitioners can deploy separate models in various situations to improve the overall performance across the board. 


\vspace{1mm} \noindent \textbf{Impact on NLP Researchers.} For academia, this also provides an impact for future research. Maybe for complex problems in the NLP domain, a single model is not the best solution and a combination of multiple models could lead to better overall performance and drive state of the art models to higher levels. 

This also includes the previous work done on unsupervised model selection. Previous researchers have implemented different techniques all leveraging different aspects of machine learning validation. Some techniques look at how similar the hidden representations to determine how similar the datasets are, and some use probability of a sample belonging to the source. Our ensemble model is the first to our knowledge that combines the strengths of all aspects of the different techniques into a single measure to estimate performance. Leveraging the different methods can help change the direction of unsupervised model selection since the methods we investigate and implement are not exhaustive. 


==> Sections/Experiments.tex <==
\section{Experiments}

In order to address and test whether the hypothesis are supported, we ran multiple experiments and analyzed performance across the 15 cities in the GeoOLID dataset. In the next two subsections, we restate each hypothesis, provide the evidence to support it, and finally provide a discussion around the results, summarizing major implications.



%In Table \ref{tab:OLID-results}, the precision, recall, F1, and accuracy shown, is the average validation results between every word embedding and random seed used during training.
{\color{blue}

%\vspace{1mm} \noindent \textbf{Geographic Performance}
%With all of the models trained and fine-tuned on OLID, we can now perform inference on the GeoOLID dataset. We predict the annotated label, Offensive or Not Offensive, for each city for every trained model with every random seed. This allows us to measure how performance changes across the different locations and where performance is not equal. For each city, we use the best model in each category and take the average performance across all seeds. This measure is reported in Table \ref{tab:city_pred}, and the best overall architecture is bolded in order to highlight the fact that the best model for each city differs. 

%In parallel with this study, we also measure the correlation of accuracy for each city. In Figure \ref{fig:correlation-ACC}, the correlation of all models, e.g., ranking all models for each city and checking correlation is shown. This is another approach to measuring the performance differences across the different cities.
}






==> Sections/Future.tex <==
With a gap in research around measuring geographic disparities in text classifiers, this is just an introduction into a branch of research focused on how locational differences affect the performance of a classifier. We believe there are a plethora of ways to extend the research presented in this paper, and begin to further improve the performance of NLP classifiers.

With our GeoOLID dataset, we now provide researchers the capability to work with locational text data. In future work, we plan to implement different methodologies of how to select the best models based on the differences in content and style of text from that location. The best overall model is the LSTM with an average accuracy of .815 across all cities. If instead of using a single model, and had an method of selecting the best model, we could potentially increase the overall accuracy of the entire text classification system.

With the the evidence supporting the different hypothesis of how location can affect performance, this can extend current research in fairness and bias in machine learning. Typically fairness is done in terms of protected attributes such as race, gender, sexual orientation, but this research and the dataset presented allows research to improve locational fairness and bias in machine learning. 



==> Sections/Hypoth.tex <==
%\section{Hypothesis and Results}

\subsection{Data Collection Evaluation}


%With our exploratory data analysis done on GeoOLID and training classifiers to predict offensive language on twitter, we feel we provide enough evidence to support all the hypothesis.



%Discuss PCC






%Discuss Prediction of City




In this section, we aim to measure how well the GeoOLID dataset matches the original unfiltered data from each city.%we address hypotheses H1a and H1b. More specifically, we analyze how different the stylistic and content differs across each of the 15 cities in the GeoOLID dataset. Moreover, we look at the correlation between language style and the demographic makeup of each city.


\noindent \textbf{Methods.} To address these hypotheses we make use of two distinct methods. First, to answer H1a, we train a geolocation prediction model. Given a tweet, the goal of the geolocation model is to predict the city in which the text was posted. To train the model we use two sets of features: Content Features and Stylistics Features. The content features are made up of the top 5000 unigrams in the unlabeled GeoOLID dataset. The goal is to ensure that common content information is used, while avoid highly location-specific terminology. We also explore two sets of style Features: Part-of-Speech and Dialect Features. Specifically, we use unigram, bigram, trigram POS features. Moreover, the dialect features are the probabilities returned from the dialect inference tool from \citet{blodgett2016demographic}. Given a tweet, the tool outputs the proportion of African-American, Hispanic, Asian, and White topics. The paper shows that the African-American proportions correlate with AAE language features. Finally, we train a Random Forest classifier on the unlabeled GeoOLID dataset and the results are reported using the labeled GeoOLID dataset as the test set. Hyperparameters are optimized using 10-fold cross-validation on the training data.


Second, to answer H1b, we we use the dialect information from the dialect inference tool from \citet{blodgett2016demographic} and correlate it with the demographic information of each city. Specifically, using the 2020 US Census data, we calculate the proportion of ``Black or African American alone'' (AA) and ``Hispanic or Latino'' (H/L) residents for each city. We also calculate the average African-American (AAS) and Hispanic (HS) topic proportion for each city using the tool from \citet{blodgett2016demographic}. Finally, we calculate the Pearson Correlation Coefficient (PCC) between the proportion of AA and H/L residents in each city.


\vspace{1mm} \noindent \textbf{H1a: Text in GeoOLID is distributed differently depending on the location it was posted.}
%In our section that describes the makeup of our novel dataset GeoOLID, it becomes apparent that text on social media truly is distributed differently depending on the location it was posted.
The results for the experiments addressing H1a are reported in Table~\ref{tab:city_pred}. Using content and style features, we were able to predict the location of a tweet more than 38\% of the time, an increase of almost 140\% in accuracy than the best random baseline, suggesting that both content and style features are predictive of the location a tweet is made. 
Likewise, using the POS and dialect features alone, the model achieves an accuracy of more than .35, substantially higher than the random baselines. Given that there are only four dialect features, this is indicative that the group information detected by the \citet{blodgett2016demographic} is informative. Similarly, the POS results are also high, indicating that there are unique combinations of POS patterns that appear in each location. Overall, the findings point to the fact that there are unique stylistic and content-related differences in each location which is important for supporting Hypothesis H2 about variations in model performance across different locations.
%More specifically, a combination of BoW and Dialect produced the best model in terms of Accuracy and F1 scores. This model is almost a 139.421\% gain in performance than using the best Random Baseline.
%This, in combination with the PCC, are important pieces of our research as in it supports the claim there are truly differences between style, content, and language between geographical locations (cities).

%Topic distribution also shows that content of social media posts vary across geological locations. Looking at Figure \ref{fig:geo-map}, we map the total number of tweets that are "border-related". As you can see, states that boarder other countries are more likely to talk about border issues than the states found in the Midwest. States like Texas, California, New Mexico and Arizona have higher proportions of these tweets and board Mexico. This further provides support to the hypothesis H1a. Topics can vary across depending on where the tweet was posted. 

%In another approach to measure the geographical disparities in our dataset, we train multiple models to classify the location of a tweet into one of the 15 cities. A logistic regression using content vs stylistic features, like Bag of Words (BoW), Part of Speech tags (POS) and the Dialect of the tweet (AAE vs SAE), attempts to  classify every tweet in the dataset into the correct city of origination. In addition to the  content vs stylistic we aslo tested different combinations of the three. For the training step we split the tweets into a traditional 80/20 split and report the F1 and Accuracy on the train set.



\begin{table}[t]
\centering
\resizebox{0.85\linewidth}{!}{%
\begin{tabular}{lrrrrr}
\toprule
                 & \textbf{AAS} & \textbf{HLS} & \textbf{Tot.} & \textbf{AA} & \textbf{H/L} \\ \midrule
\textbf{Bal}    & .168     &    .193     & 585,708    & 338,478       &  45,927         \\
\textbf{Chi}      &         .147   &  .204 & 2,450,143  & 801,195       & 819,518          \\
\textbf{Col}     & .146    &     .201     & 905,748    & 259,483       & 70,179          \\
\textbf{Det}      & .196   &     .214     & 639,111    & 496,534       & 51,269          \\
\textbf{ElP}         & .158  &    .227       & 678,815    & 25,077       & 551,513          \\
\textbf{Hou}     & .161  &      .205      & 2,304,580  & 520,389       & 1,013,423          \\
\textbf{Ind} & .151      &   .194     & 887,642    & 248,067       & 116,221          \\
\textbf{LA}    & .144    &      .204    & 3,898,747  & 336,096       & 1,829,991          \\
\textbf{Mem}     & .209       &   .220    & 633,104    & 389,779       & 62,167          \\
\textbf{Mia}       & .140  &     .175       & 442,241    & 57,254        & 310,472          \\
\textbf{NO}    & .182       &    .197   & 383,997    & 208,273       & 31,017          \\
\textbf{NY}       & .126    &     .182     & 8,804,190  & 1,943,645     &  2,490,350          \\
\textbf{Phi} & .157      &    .204    & 887,642 & 248,067       & 116,221          \\
\textbf{Pho}      & .144   &    .208       & 1,608,139  & 125,260       & 661,574          \\
\textbf{SA}     & .175    &     .222     & 1,434,625  & 102,816       & 916,010          \\ \midrule 
\textbf{AA PCC} & \multicolumn{4}{c}{.565 (\textit{p} value: .028)} \\ 
\textbf{H/L PCC} & \multicolumn{4}{c}{.167 (\textit{p} value: .55)} \\ \bottomrule
\end{tabular}%
}
\caption{Pearson Correlation Coefficient (PCC) between the AAS and HLS.  The abbreviations for the 15 cities in the GeoOLID dataset are as follows: Chicago~(Chi), Detroit~(Det), Baltimore~(Bal), El Paso~(ElP), Los Angeles~(LA),  Houston~(Hou), Columbus(~Col), Indianapolis~(Ind), Miami~(Mia), Memphis~(Mem),  New York City~(NYC), New Orleans~(NO), San Antonio~(SA), Philadelphia~(Phi),  and Phoinex~(Pho).\vspace{-2em}}
\label{tab:PCC}
\end{table}


\vspace{1mm} \noindent \textbf{H1b: Text made in certain geographic regions is representative of the sociodemographic makeup of the area.} In addition to the classification of a tweets location, we present a strong correlation between the sociodemographic makeup of each city and the dialect style of the tweets within the dataset. If a cities population of residents has a higher percentage of African Americans, then prior work has shown that there is an increase in the number of occurrences of AAE-related language patterns~\cite{blodgett2016demographic}. Specifically, using the average AAE (AAS) and Hispanic (HLS) scores from the \citet{blodgett2016demographic} tool over all tweets in each city, we correlate it with the proportion of AA and Hispanic population within each city based on the 2020 US census data. This correlation can be seen in Table \ref{tab:PCC}. Overall we find that there is significant correlation .565 ($p$ value: 0.028) between the two variables. We find that cities like Baltimore, New Orleans and Detroit are more likely to have more AAE tweets then cities like Miami, Columbus, and New York. For the Hispanic group we also find a positive correlation but the finding is not significant. We also manually analyzed the dataset and found other features indicative of a relationship between demographics of the city and language use. For example, we found Spanish curse words appearing in text in cities with higher Hispanic populations in our dataset, e.g., ``Nationwide shutdown! pinché Cabron'' is an slightly modified tweet that appeared was tagged in Phoenix, AZ.


%{\color{red} Rios, Maybe you can talk about MDE here as well.}

%{\color{red} Maybe show spanish examples as well}

\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrrrrrrrrrrrr}
\toprule
       & \textbf{Bal} & \textbf{Chi} & \textbf{Col} & \textbf{Det} & \textbf{ElP} & \textbf{Hou} & \textbf{Ind} & \textbf{LA} & \textbf{Mem} & \textbf{Mia} &  \textbf{NO} & \textbf{NY} & \textbf{Phi} & \textbf{Pho} & \textbf{SA} & \textbf{AVG} \\ \midrule
\textbf{Stratified} & .555 & .555 & .550 & .536 & .536 & .570 & .577 & .567 & .521 & .592 & .553 & .588 & .567 & .544 & .564 &  .558 \\
\textbf{Uniform}    & .484 & .533 & .500 & .510 & .465 & .504 & .479 & .477 & .487 & .484 & .495 & .509 & .503 & .503 & .513 &  .496 \\
\textbf{Prior}      & .695 & .675 & .672 & .599 & .554 & .681 & .662 & .689 & .605 & .771 & .651 & .730 & .651 & .618 & .596 &  .657 \\ \midrule \midrule
\textbf{NB}         & .820          & .765        & .779         & .764        & .695        & .781        & .773             & .794            & .769        & .863      & .787        & .797         & .782             & .710        & .743     &    .775   \\
\textbf{Linear SVM} & .779          & .745        & .751         & .761        & .694        & .724        & .748             & .776            & .752        & .822      & .787        & .794         & .771             & .704        & .740        &   .757 \\ \midrule
\textbf{BiLSTM}    & .834 & .809 & \textbf{.799} & .803 & .757 & .774 & .809 & .824 & \textbf{.818} & .861 & .835 & .842 & .833 & .768        & .783 &   .809  \\
\textbf{CNN} & \textbf{.843} & \textbf{.820} & .792 & .823 & .747 & .773 & \textbf{.819} & .805 & .814 & .851 & \textbf{.842} & \textbf{.849} & .849 & .760 & \textbf{.788} &   .811  \\
\textbf{LSTM}       & .832 & .814 & .790 & \textbf{.834} & \textbf{.758} & .790 & .817 & \textbf{.829} & .810 & \textbf{.873}      & .837        & .834         & \textbf{.850}             & \textbf{.772}        & .783       &    \textbf{.815} \\
\textbf{BERT}       & .786             &  .800          & .788            & .785           & .755           & \textbf{.791}           & .790                & .809              & .761           & .848         & .785           & .816            & .803                & .747           & .771         &     .739 \\ \midrule
\textbf{AVG} & .816 (0) & .792 (1) & .782 (1) & .795 (1) & .734 (8) & .772 (1) & .793 (1) & .806 (1) & .787 (1) & .853 (0) & .812 (2) & .822 (0) & .815 (0) & .744 (6) & 	.768 (2) & \\ \bottomrule
\end{tabular}%
}
\caption{Accuracy. In the bottom row, we mark the number of other cities that have a score greater than or equal to the MDE for that city given its score as a baseline.\vspace{-2em}}
\label{tab:City-ACC}
\end{table*}

\begin{table}[t]
\centering
\resizebox{0.55\linewidth}{!}{%
\begin{tabular}{lrr}
\toprule
       & \multicolumn{2}{c}{\textbf{PCC}} \\ \cmidrule(lr){2-3}
       & \textbf{AA}         & \textbf{Hispanic}       \\ \midrule
\textbf{NB}         & .186  & -.216    \\
\textbf{Linear SVM} &  .142  & -.272    \\
\textbf{LSTM}       &  .279  & -.362    \\
\textbf{CNN}        & .283   & -.398    \\
\textbf{BiLSTM}     &  .290  & -.358    \\
\textbf{BERT}       & -.061   & .056     \\
\textbf{AVG}        &  .187  & -.258 \\ \midrule \midrule
\multicolumn{3}{c}{\textbf{AAE vs SAE Results}} \\ \midrule
\textbf{SAE Accuracy}  & \multicolumn{2}{c}{.831} (3392) \\ 
\textbf{AAE Accuracy}  & \multicolumn{2}{c}{.854} (5789) \\ \midrule
\textbf{SAE FPR}  & \multicolumn{2}{c}{xxx} (3392) \\ 
\textbf{AAE FPR}  & \multicolumn{2}{c}{xxx} (5789) \\ \bottomrule
\end{tabular}}%
\caption{PCC between AA and H/L population proportions of each city and Accuracy. This table also reports the SAE vs. AAE Accuracy/FPR on the GeoOLID dataset---the total number in each group is in parenthesis.\vspace{-2em}}
\label{tab:per-cor}
\end{table}

\subsection{Data Variation and Model Performance}
\label{sec:var}

In this subsection, we explore the central hypotheses of this paper looking at performance disparities between various locations within the US.


\noindent \textbf{Methods.}
We train six different machine learning algorithms: Naive Bayes (NB), Linear Support Vector Machine (Linear SVM), Long Short Term Memory (LSTM), Bidirectional LSTM (BiLSTM), Convolutional Nueral Networks (CNN), and a Bidirectional Encoder Representations from Transformers (BERT). Each model is trained to classify Offensive and Non Offensive tweets using the OLID dataset.% on each of the five training OLID training splits. With multiple trained models on the OLID data, we can then do inference on the GeoOLID tweets and find the best model for every city as well as the performance disparities. 
Each model is trained independently on each of the five different OLID training splits. The performance metrics are then averaged across the five different seeds as a way of measuring the robustness of the model and guaranteeing a high accuracy is not a coincidence when predicting on the same validation set.
%In Table \ref{tab:OLID-results}, we take the average of the 5 independent prediction results and report the average overall accuracy on the validation set.
One thing to note is for the BiLSTM, CNN and LSTM, we also measure the performance of the model across multiple word embeddings. Specifically, each deep learning model is trained using different variations of Glove, Google Word2Vec and Fasttext word embedding (See the Appendix for a complete listing of the evaluated embeddings). We also perform a comprehensive manual error analysis for H2b to better understand model performance differences beyond aggregate quantitative metrics.


\vspace{1mm} \noindent \textbf{H2a: Because data is distributed differently in different geographic regions, model performance is not the same in each location.} In Table~ \ref{tab:City-ACC}, we report the OLID model accuracy for each city. Overall, we find substantial variation in model accuracy across the 15 cities. The Naive Bayes (NB) classifier ranges from .695 to .863, resulting in around a 17\% difference in accuracy between El Paso and Miami. Similar findings can be seen with the other models like CNN and BERT having a up to a 10\% difference. Furthermore, given the MDE of around 5\% for each city depending on the baseline score, we find that many of the differences are significant. Note that there are even larger differences in F1 score, please find the results in the Appendix.



The question remains, if the text in each city is correlated with demographic information, then why do we need location-specific performance analysis? The issue is that while demographic analysis provides broad insights, location-specific language is substantially more varied. Thus, unfortunately, demographic factors alone are not predictive of model performance for a given city. In Table~\ref{tab:per-cor}, we use the \citet{blodgett2016demographic} tool to identify AAE and SAE (White-aligned) tweets in our GeoOLID dataset across all cities. When we calculate the false positive rate (FPR) across these two aggregate groups, we find similar conclusions to prior work~\cite{sap2019risk} suggesting that offensive language models are biased towards AAE text. However, when we correlate (using PCC) model performance (Accuracy) with the proportion of Black or African American residents using US Census data, we find that the model is positively correlated (though not significant) with higher accuracy, which is contrary to the general demographic findings. We also correlate the performance of each model with Latino or Hispanic populations finding negative correlations. After manual analysis, we find that the models suffer for common topics in these areas (e.g., border-related topics). In summary, the major finding of this paper is listed below:
%\setlength{\fboxsep}{0pt}
%\setlength{\fboxrule}{0pt}
\begin{center}
\noindent\fbox{%
    \parbox{.93\linewidth}{%
        \textbf{Major Finding:} Broad dialectal analysis of model performance alone is not predictive of model performance for a specific community.
    }
}
\end{center}

%\noindent Hence, we 

%In addition to looking at the range of accuracies for each model, Figure \ref{fig:correlation-ACC} shows the correlation between overall accuracy and every city. If performance was constant, regardless of the city, we would see very similar shades of blue across the entire correlation map. In the figure, the shades of blue vary from dark blue to white, and supports the hypothesis that perfromance can vary with locations. 

%\vspace{1mm} \noindent \textbf{Downstream Task:}


\vspace{1mm} \noindent \textbf{H2b: Errors made by the models are caused by geographic-specific content and language style.}
\begin{figure} 
    \centering
    \includegraphics[width=\linewidth, height=4.5cm]{error_analysis.pdf}
    \caption{Category Percentages of False Negative Predictions per City.\vspace{-2em}}
    \label{fig:error_analysis_FN}
\end{figure}
We perform a comprehensive manual analysis on the false negatives made by the best model on the OLID dataset. Specifically, we performed a qualitative open coding procedure to categorize the false negatives into commonly occurring groups. The first author of the paper conducted a preliminary analysis on a completely random sample of XXX false negatives, identifying the main codes. Next, a meeting was help where the main codes were discussed and. The final group of codes were identified as: Racist, Profanity, Targeted, Inappropriate, and Other. Following the meeting, both the first author and a coauthor coded a total of XXX false negatives (100 for each city) achieving an agreement of XXX.

The results are summarized in Figure~\ref{fig:error_analysis_FN}. Specifically, we categorized false negatives into four major categories: Racist, contained profanity, was a target attack on an individual, or was inappropriate (sexual references, insensitive jokes). A few important observations can be made from this graph. For instance, we find a large proportion of false negatives in the racist category in border cities, or cities in close proximity to Mexico (e.g., El Paso, Phoenix, San Antonio, and Houston). We found many issues where the model did not detect language that refers to migrants being part of a ``horde,'' meant to cause violence or destruction (this is common racist rhetoric at the time~\cite{finley2020immigrant}),  as being offensive. Given the increase in border-related topics, this type of error is highly location-specific.
Furthermore, non-location-specific errors include compound curse words and morphological variants of curse words that were a major cause for false negatives in multiple regions. For example, in New Orleans,  Philadelphia, and Memphis there were many false negative tweets contain high percentages of Profanity due to multiple spellings of different swear words such as phucking, effing, mothafucka, biatches.% These types of phonics are highly correlated with AAE dialects and with these cities having high proportions of African American residents, this also supports the Hypothesis. 


\subsection{Geographic Similarities}

In this subsection, we analyze the correlation between the best performing models in each city. %Specifically, we answ Is the best model the same in each city? does optimizing the performance of a model on data in New York also improve the performance


\noindent \textbf{Methods.} To answer this question, we analyze the performance of the models trained and described in Section~\ref{sec:var}. Specifically, we compare the PCC between the Accuracy of each applied for every pair of cities. Intuitively, if the rank of each model for New York based on Accuracy is the same as the rank of each model applied to Phoenix, then the correlation would be one. The more differences in rankings the lower the performance. In this experiment, we rank every model along with the variants of models (i.e., each model trained with different word embeddings listed in the Appendix are treated as independent models).


\vspace{1mm} \noindent \textbf{H3: The best model for each location is not the same.} The results of the correlation analysis are shown in Figure~\ref{fig:correlation-ACC}. Overall, similar to variations in model performance across cities, we find that the similarity in model performance correlations can vary substantially city-to-city. For instance, the best models for Houston are substantially different than other cities with the exception of a few (e.g., Los Angeles). However, on further inspection, general architecture performance seems to be relatively similar across cities, e.g., the LSTM model is the best on OLID dataset and for most cities. Much of the variation comes from hyperparameter choice , or more specifically pretrained embedding choice(with more than 10\% in Accuracy between the best and worst embeddings). This suggests that choosing the best hyperparameters based on a small subset of data is not optimal for each community. An interesting future research question would be if we train a model with many hyperparameter options on a dataset, is it possible to predict which model to deploy in a given region?


%{\color{red} Still need to provide some analysis on the table and look for other patterns}}



%This section  three major experiments and analysis: correlation, best classification choice, and cross-dataset similarities.

%{\color{red} Lets get results for F1 as well to address part of the reviews. Also, lets expand the discussion about bias results. Lets add a manual error analysis subsection.}

%{\color{red} Need to still talk about Figure 2. Correlation}

\begin{comment}
\begin{table}[t]
\centering
\resizebox{.7\linewidth}{!}{%
\begin{tabular}{lrrrr}
\toprule
           & \textbf{Prec.} & \textbf{Rec.} & \textbf{F1} & \textbf{Acc.} \\ \midrule
           \multicolumn{5}{c}{\textbf{Random Baselines}} \\ \midrule
\textbf{Stratified} &   .324 & .348 & .336 & .553          \\
\textbf{Uniform}    &     .321 & .505 & .392 & .493         \\
\textbf{Prior}      &    .000 & .000 & .000 & .676         \\ \midrule \midrule
\multicolumn{5}{c}{\textbf{Machine Learning Models}} \\ \midrule
\textbf{NB}         &         .722  & .250       &  .371  &     .720     \\
\textbf{Linear SVM} &        .643 & .505       &  .566  & .744          \\ \midrule
\textbf{BiLSTM}     &       .754    &   .551     &  .635  &      .792    \\
\textbf{CNN}        &       .721 & .603       & .655   &    .790      \\
\textbf{LSTM}       &     .768      &   .527     &  .625  &    .791      \\
\textbf{BERT}        & .652 & .555 & .592   &  .752        \\ \bottomrule
\end{tabular}%
}
\caption{OLID Results\vspace{-1em}}
\label{tab:OLID-results}
\end{table}
\end{comment}


\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{accuracy_correlations.pdf}
    \caption{Model accuracy correlation between each pair of cities in GeoOLID.\vspace{-2em}}
    \label{fig:correlation-ACC}
\end{figure}



%\begon{comment}
%\textbf{NB}         & -.064   & -.216    \\
%\textbf{Linear SVM} & -.281   & -.272    \\
%\textbf{LSTM}       & -.364   & -.362    \\
%\textbf{CNN}        & -.429   & -.398    \\
%\textbf{BiLSTM}     & -.395   & -.358    \\
%\textbf{BERT}       & -.019   & .056     \\
%\textbf{AVG}        & -.259   & -.258 \\ \bottomrule
%\end{comment}

==> Sections/Intro.tex <==
%1. models don't generalize 

%\textbf{Paragraph 1}: State the problem/task and its importance (i.e., geographical bias of classifiers)%

Text classification, especially when applied to social network data or online blogs, has been applied to wide array of tasks including, but not limited to tracking viruses~\cite{lamb2013separating,corley2009monitoring, corley2010text, santillana2015combining, ahmed2018social, lwowski2020covid}, providing help for (natural) disasters~\cite{neubig2011safety,castillo2016big,reuter2018fifteen}, detecting misinformation~\cite{oshikawa2020survey}, and identifying cyber-bullying~\cite{xu2012learning}. Overall, text classifiers have been shown to be ``accurate'' across a wide range of applications. As deep learning models and packages have made substantial progress for the field of natural language processing (NLP), NLP models have become more accessible to the general public. Hence, models are being deployed in a production environment and ran at scale at a growing pace. However, recent work has shown that these models are biased and unfair, especially towards minority groups~\cite{blodgett2016demographic,davidson2019racial}. In this paper, we expand on prior work by analyzing how model performance can fluctuate due do geographical-caused differences in language and content that may exist in the context of offensive language detection.

%\textbf{Paragraph 2-3}: Describe major prior work looking at similar issues (e.g., differences in performance between dialects and languages) and what they found.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{usa.pdf}
    \caption{Proportion of border-related tweets in the GeoOLID dataset~\cite{qazi_geocov19_sigspatial} for each state.\vspace{-2em}}
    \label{fig:geo-map}
\end{figure}

% Both language style and content can be unique between different geographical locations. Cities that boarder the Mexico and the United States could have Spanish words intertwined with English or cities with high percentages of
% When comparing cities, distribution of topics can differ greatly depending on the make up of the city. A city like Los Angeles may have more mentions of sports due to the large amount of profession teams located in that city, or maybe the general political stance of city could differ greatly when looking at different geographical regions.

% schlechtweg2019wind

Several lines of research have shown that topical and stylistic attributes of text are used by speakers on social media to implicitly mark their region-of-origin~\cite{shoemark2017topic, hovy2018capturing, hovy2020visualizing, cheke2020understanding, gaman2020report}. For instance, \citet{hovy2018capturing} show that doc2vec embedding frameworks which can be used to can help with the task of geolocation prediction. \citet{hovy2020visualizing} then introduces visualization techniques for measuring regional language change. \citet{kellert2021geolocation} shows that these differences exist at the city level as well. Our data consists of geo-tagged COVID-related tweets. In Figure~\ref{fig:geo-map}, we measure the proportion of border-related tweets in each state to show case how topical content can be distributed geographically, finding most of the border-related tweets are in states near Mexico (e.g., Texas, Arizona, New Mexico, and California). Overall, much of the prior work has focused on better incorporating or identifying regional aspects of language data to improve performance in machine translation~\cite{ostling2017continuous} or geolocation prediction~\cite{hovy2018capturing}.

Recent work in understanding performance disparities has found differences across various languages~\cite{gerz2018relation} (e.g., Finish vs Korean) and dialects~\cite{davidson2017automated,sap2019risk}---such as African American English (AAE)---can have a substantial impact on model performance. For instance, \citet{gerz2018relation} show that fine-grained typological features must be incorporated into language modeling architectures for a single model to adequately perform across a wide array of languages. More specifcally, the absence of typological features is predictive of substantial performance disparities across languages. Likewise, \citet{davidson2019racial} and \citet{sap2019risk} show that abusive and hate speech-related language classifiers are biased against AAE-like text. These results have been shown to extend into other text classifications tasks, for example, \citet{lwowski2021risk} show that influenza detection models are also biased against AAE-like text. These findings show that models deployed at scale can adversely impact minority groups.

%\textbf{Paragraph 3-4}: State the research gap in prior work (e.g., No work on Geographical differences in performance)
Overall, while there has been a substantial amount of research understanding how to identify and use regional (geographical) features and identify performance disparities across languages and dialects, to the best of our knowledge, there has been no prior work understanding geographical performance disparities across regional dialects. Do regional language differences, whether content or language style, impact offensive language model performance? While prior work has shown that dialect can impact, and dialect is correlated with social demographics of regional areas~\cite{blodgett2016demographic}, . For instance, AAE is not spoken the same in every region of the United States (US). There are well-known sub-dialects such as Rural and Urban AAE. But, more importantly, certain features of AAE only appear within specific regions of the US~\cite{jones2015toward}. Does the interaction between AAE features and content spoken in one region adversely impact model performance more than other regions? There has been extensive research, understanding geographical health disparities, which are thought to be due to limited physical access to health care, but also to differences in demography, attitudes, lifestyle factors, and cultural practices in regional and rural settings~\cite{eberhardt2004importance,smith2008addressing,dixon2000researching}. Prior work has shown that performance disparities can potentially increase health disparities for minority communities~\cite{lwowski2021risk}. Hence, depending on the applications in which text classifiers are applied (e.g., offensive language), geographical algorithmic disparities can further harm (e.g., the mental health) these regions.

%It is unknown whether these geographical differences can impact models developed for real-world tasks such as offensive language detection. studying geographical differences in textual data has been deeply explored, there seems to be a major research gap in understanding how performance is effected by these differences and is an one model fits all the best solution to at-scale NLP classifiers. Fairness and discovering biases of classifier is a common practice and measures performance gaps between different sub-populations \cite{lwowski2021risk} but, to our best knowledge, there is a lack of research around training multiple classifiers for the same task and measuring the performance metrics across different geolocations.

%\textbf{Paragraph 4-5}: State what we will do to overcome the research gap

% Is the dataset used for training representative of the differences of dialect, style and content present in varying locations? Does selecting a certain model or word embedding improve the performance for different sub populations? Which model should we deploy in different parts of the country? These are the types of problems that arise when investigating the differences in performance across a diverse geographical region. 
To better understand the implications of geographical performance disparities, we make three major contributions:
\begin{enumerate*}[label=\bfseries (\arabic*.)]
\item We introduce a new dataset called GeoOLID with more than 13 thousand tweets across 15 geographically and demographically diverse cities in the United States.
\item We produce a comprehensive dataset analysis, analysing both the content and stylistic variations in each city.
\item Finally, we perform a comprehensive analysis of performance disparities across a wide array of popular text classification models in each city, producing novel insights and discuss important future avenues of research.
\end{enumerate*}

% we train multiple classifiers to identify offensive language on twitter based on the previous work of \citet{zampieri2019predicting}. We then apply the trained classifiers to predict offensive language of tweets collected from 15 different cities across the United States during the Covid-19 pandemic. This allows us to measure the geographical disparities across different locations with multiple machine and deep learning models. 

%Final Paragraph: Summarize research questions/hypothesis of this paper 

%Overall, the contributions of this paper can be summarized as follows:
%\begin{enumerate*}
%\item We introduce a new dataset (GeoOLID) with nearly 14 thousand ...
%\item We perform a comprehen.
%\item 3
%\end{enumerate*}

\begin{comment}
{\color{blue}
In order to address the research gap in performance differences across geographical regions, our contributions include testing the following hypothesises:
\vspace{-.1em}
\begin{itemize}%[start=1,label={\bfseries H\arabic*):},align=left,widest=ii, labelsep=0pt,leftmargin=*]
\itemsep-.5em 
\item[\textbf{H1a.}] Text on social media is distributed differently (based on content and style) depending on the location it was posted. 
\item[\textbf{H1b.}] Text made in certain geographic regions is representative of the sociodemographic makeup of the area.
\item[\textbf{H2a.}] Because data is distributed differently in different geographic regions, model performance is not the same in each location.
\item[\textbf{H2b.}] Errors made by the models are caused by geographic-specific content and language style. (Maybe error analysis can help address this)
\item[\textbf{H3.}] The best model for each location is not the same.
\end{itemize}
\vspace{-.1em}
Lastly, we introduce a English US-centric dataset of offensive language collected across fifteen geographically, and demographically diverse cities called GeoOLID in order to allow researchers to continue the work in measuring performance differences across diverse populations.
}
\end{comment}


\begin{comment}
{\color{red} Read the review and update the intro addressing their concerns, e.g., remove part about saving computation, make aspects more clear, etc.}

Model deployment is a continuous process that does not finish after training a model for a specific task. It is widely accepted that machine learning-based natural language processing models do not generalize from the \textit{source} dataset to examples from different domains (the \textit{target} data) because of issues with ``shifts''' in the data. Specifically, models can go ``stale'' over time because of \textit{covariate shift} (i.e., changes in the features over time)~\cite{kim2017adversarial,blitzer2007domain,storkey2009training}, \textit{label shift}~\cite{lipton2018detecting} when the proportion of certain topics/classes change over time, and \textit{concept shift} when the inherent meaning of classes change. In practice, models may go ``stale'' slowly over time as the topics discussed in the training dataset change, or in an instant because of deployment needs. A large internet company may develop a model for a specific task and expect to deploy it to all of their customers in a given country (e.g., the United States). Nevertheless, because of the high cost to curate large datasets, the training dataset will only cover a fraction of the population that the model will impact. Thus, the model may not generalize to all regions of the deployment area because of instant ``shifts''.
%For example, ``y'all" is widely used in Texas, but might not be significant in the distribution of vocabulary in New York city.

There have been a wide array of approaches to handle various ``shifts'', many of them work on the assumption that the target data is devoid of labeled data (unsupervised domain adaptation). Traditional methods re-weight training instances based on their similarity to the target dataset~\cite{shimodaira2000improving,jiang2007instance,ben2010theory,sun2019unsupervised, shen2018wasserstein, pinheiro2018unsupervised}. For example, \citet{jiang2007instance} used an instance weighting-based approach for text. They remove source instances that are significantly different from the target data. \citet{daume2007frustratingly} used a feature augmentation method with special features for the source and target data, as well as shared feature representations for both. \citet{ganin2015unsupervised} developed an adversarial domain adaptation technique for neural networks. \citet{kim2017adversarial} expand on the use of the adversarial adaptation method to adapt neural networks in the presence of temporally-caused covariate shift. Overall, while many methods have been proposed to handle ``shifts'', many methods are challenging to train and require substantial ``hand-holding'' to optimize precisely. For instance, adversarial domain adaptation methods are unstable and require ``regularization tricks'' during training~\cite{mao2017least,chen2020adversarial,rios2018generalizing}. Thus, applying unsupervised domain adaptation methods at scale may be infeasible.

Other major challenges with unsupervised domain adaptation methods involve the question, ``How should the hyperparameters be chosen if we assume the target data in unlabeled?'' The best hyperparameters on the source dataset may not necessarily result in the best parameters on the target data. Researchers have introduced a broad set of methods under the umbrella of unsupervised domain adaptation model selection to answer this question. For instance, \citet{pmlr-v97-you19a} recently proposed an unbiased estimation of the target performance, expanding on the importance weighted validation methodology~\cite{sugiyama2007covariate}. Intuitively, both methods weight the errors on a held-out dataset based on their similarity to the target data. Nevertheless, while many of these model selection approaches have been shown to improve certain techniques' performance, there are still many unknowns about them. For instance, evaluation methodologies for these approaches focus on evaluating hyper-parameter selection (e.g., to choose the best learning rate for a single model). However, can they be used to compare models of different architectures? If we have $N$ models, each trained with $k$ hyper-parameter settings, can the model selection criteria metrics be used to rank all model--hyper-parameter combinations based on out-of-domain performance? Suppose models can be appropriately ranked, then instead of fine-tuning models unsupervised domain adaptation techniques can be used for each possible deployment area. In that case, practitioners can train many models during training (which is often done to find the best model on the source data) and predict which to deploy to each location. Reusing models can also negate some of the energy consumption used to train them~\cite{strubell-etal-2019-energy}.



In this paper, we define two main goals of model selection metrics. First, they should estimate the \textit{generic (broad) robustness} of models to out-of-domain data. Some models may generalize better than others. A robust model selection metric should be able to rank general robust methods higher than domain-sensitive models, i.e., it should answer the question ``on average, which models are most robust to distributional shifts?'' Second, no model will generalize equally to all data shifts. Thus, we test whether these metrics can \textit{measure fine-grained differences} in shifts to domain change. For instance, the metrics should answer the question, ``which models work better on data collected from Chicago?'' To answer these questions, we collected and annotated more than 16k English tweets from fifteen geographically diverse US cities for the task of offensive language detection. We compare state-of-the-art unsupervised domain adaptation metrics for each city and an interesting combination of multiple metrics. Moreover, we analyze the impact of simply using a completely out-of-domain dataset to rank the performance of models across all cities.


Overall, the contributions of this paper are summarized as follows:
\begin{enumerate*}[label={(\bfseries \arabic*)}]
    \item We introduce a English US-centric dataset of offensive language collected across fifteen geographically, and demographically diverse cities called GeoOLID for the novel task of fine-grained unsupervised model selection. The purpose of the dataset is to facilitate the novel development of fine-grained unsupervised out-of-domain model selection criteria.
    \item We provide a novel evaluation framework for comparing that model selection metrics using ranking correlations.
    \item We provide a comprehensive evaluation of state-of-the-art methods and several unique baselines for the dataset. Moreover, we evaluate several simple combinations of current model selection methods, providing non-trivial improvements to existing techniques.
    \item We provide a comprehensive set of recommendations for practitioners and researchers to better handle model selection in the presence of data shifts facilitated by our exhaustive evaluation procedure.
\end{enumerate*}
%2. we already train tons of models 
%In an attempt to deploy the best model into production, machine learning and nlp experts typically train multiple models with different variations and test against a holdout set. The model that performs best on the holdout set is used and deployed in production and the rest are disregarded. We argue that we should not just throw away previously trained models but instead save them for future deployment. Machine and deep learning models are financially expensive to train  and we could leverage the previously trained and tested models for personalized situational deployment. 

%By using a holdout set, researchers are trying to simulate how the model performs in the wild, with new data that it has not seen before. This method has one major downside, the holdout/validation set is typically a subset of the original dataset from a similar distribution of vocabulary words and semantics. Even though the model has not seen the data during training, the performance of the model on the validation set can give researchers and model builders a false sense of confidence on how it will perform when deployed. The data the model receives once deployed in production can be quite different than the data it was trained on and change over time.

%3. performance can suck without personalization, covariate/domain shift
%For example, if a classifier was trained to detect offensive language online and was done so using a labeled dataset that is dated, its performance will struggle to make accurate predictions on topics in today's changing online environment and vocabulary. Models trained pre-2019 would not know how to handle vocabulary like ``coronavirus" or ``covid-19" and topics/vocabulary that was not considered offensive could now be considered so. With language constantly changing, our deployed NLP models will suffer from domain and covariate shift over time, significantly impacting the performance of our classifiers. 

%One approach would be to continuously add manually annotated tweets to the dataset and retrain. This process would continue indefinitely while the model is deployed in order to guarantee that the models performance suffices for the task. This is definitely not a preferred solution. Obtaining annotated tweets is time consuming, can become expensive, and can succumb to labeling biases and errors by the annotators. 

%Another downfall to this technique is that it can suffer a decrease in performance when assuming the different sub samples of population behave and speak in the same manor. \newcite{lwowski2021risk} show that when using machine learning to classify tweets, the models performance can decrease if a users dialect belongs to a minority subclass. When training a offensive language classifier at a national level, the performance can decrease with different sub populations (different cities) talking about different topics. For example, in Chicago, sport teams like the Bears and White Sox are probably mentioned a lot more than they would be in San Antonio. And cities with different dialects use different lingo's to represent curse words and offensive language. In general, NLP models without personalization will struggle to be accurate for the various sub groups that it is deployed to. 

%4. So lets just train a bunch of models and figure out where each should be applied without labeling data for each location we want to apply it to.
%To solve the problem of choosing which model to deploy, and predicting the classifier that has the best performance at scale, we need to address the 2 issues above. It should work with unlabeled data to remove the step of paying companies or employees to continuously label data. Second, it should be personalizable to the smaller subgroup or population in order to address the covariate and domain shift between the different subgroups.

%5. Contribution: Ensemble Model using previously studied domain adaptation methods to choose the best model
%We propose a method that leverages multiple domain adaption techniques that estimates the accuracy of how classifiers will perform on out of domain data. Instead of throwing away previously trained models, we use the outputs from the techniques previously studied to train an ensemble model to choose the best model to deploy in production in various situations. We test our method on an offensive language classifier and choose the best model to deploy in 15 different cities across the United States. We show that our ensemble model outperforms selecting the best accuracy on the holdout/validation set as well as the PAD* method studied and proposed by \newcite{elsahar2019annotate}. We validate our results by using the Spearman's Rank-Order Correlation on the ordered ranking of the true best classifier vs our predicted ranking order.
\end{comment}



==> Sections/OLD_Method.tex <==

\begin{comment}
Our study has two main steps. First (\textbf{Step 1}), we train various models using different neural architectures and model parameters. We use different pre-trained word embeddings as the different model parameters. Moreover, all models are trained on the OLID dataset. We evaluate each model on the target datasets (cities in GeoOLID). Second (\textbf{Step 2}), we evaluate multiple methods of ranking performance. 

%In the method section, an in-depth explanation of the various methods used in our study is provided. In order to estimate how the classifier will perform on out of domain (OOD) data, a model must be first trained and validated on the source data. For the purpose of this study, we assume the OOD is unlabeled and are attempting to select which classifier to deploy that has the highest estimated OOD accuracy. We can then compare the estimated model rankings to the true model rankings to validate our approach.

\subsection{Step 1: Model Training}


\vspace{1mm} \noindent \textbf{Models.}
We implement three different neural network-based classifiers: a convolutional neural nets (CNN), long short term memory (LSTM), and a bi-directional LSTM (BiLSTM). For the CNN model we use the architecture proposed by \citet{kim-2014-convolutional}. 
The CNN was trained with the filter sizes of 3,4 and 5, mini-batch size of 512, and the Adam optimizer. Likewise, the LSTM-based models were trained with hidden state sizes of 512, mini-batch size 124, and Adam optimizer. All models set a max sequence length of 125 words and a max vocabulary size of 10,000 words. Also all models were ran for a max of 30 epochs with early stopping implemented.



\vspace{1mm} \noindent \textbf{Word Embeddings.}
We use three major word embedding types: Word2Vec~\cite{mikolov2013distributed, mikolov2013efficient}, GLoVe~\cite{pennington2014glove}, and FastText~\cite{bojanowski2016enriching}. For the Word2Vec word embeddings four pre-trained sets of pre-trained embeddings are used (Google News, PMC, PubMed PMC, PubMed), eight different embeddings for GLoVe (based on Twitter and Wikipedia data), and one set of FastText embeddings were used. Thus, there are a total of 39 model-embedding combinations that use use to rank model performance.



%%% TODO Add some more information here
\subsection{Step 2: Predict Model Performance}

In this subsection, we describe the methods use use to estimate target performance. Specifically, we explore six unique methods: Source, Third-Party Out-of-Domain Data, Reverse Validation (RV), Importance-Weighted Validation (IWV), and Deep Embedding Validation (DEV). We summarize each method below.

%\vspace{1mm} \noindent \textbf{Direct Method.}
%With the goal of predicting the best classifier to deploy in various situations, we use the FOUNTA, OLID and WASEEM datasets to rank the models based on how they perform on data outside of their domain. Even though the 3 datasets are similar in content they differ in what is actually being classified. Like described in the Data section, FOUNTA is abusive language, OLID is offensive language, and WASEEM is sexist and racist language. By transforming the labels of all 3 datasets into a binary task of Offensive vs Not Offensive, we can measure the performance of the various classifiers when they experience covariate and label shift. 

%For the 3 datasets, every permutation of model and word embeddings mentioned above is trained on one of the datasets, which we call the source dataset and performance is measured against the out of domain datasets. The source dataset is split into train, test, and validation and trained on 5 different random seeds in order to generalize the results. The same validation set is used on all 5 seeds in order to improve consistency. 

%Once every model, embedding, and seed are trained, it is scored against the out of domain data and their corresponding labels. A ranking order is established, ordering the model/wordembedding combination based on its true accuracy on the out of domain data. This allows for situational deployment and promotes model reuseability. For example, the best model embedding combination trained on the FOUNTA dataset and deployed for OLID is different then the combination deployed for WASEEM.  

\vspace{1mm} \noindent \textbf{Source.}
The simple method of estimating target performance is to simply use the performance on the source data. Intuitively, this is the standard assumption by model builders, i.e., that they model will generalize once deployed. Formally, we use the performance on the source data $s^{\mathcal{M}_i}$ using model $\mathcal{M}_i$ to estimate it's performance on the target dataset $\hat{r}^{\mathcal{M}_i}_j$. 
%The first way to select which model to deploy is the most used technique for model selection. Most machine learning engineers and model builders select their best model based on how the model performs on the holdout/validation set. The assumption is that the model that performs best on data it has not seen before will also perform well when deployed. Like we mentioned before, this is not always a good way of measuring performance due to the data the model receives once deployed can differ from what it was trained on. 

\vspace{1mm} \noindent \textbf{Third-Party Out-of-Domain Data.}\footnote{The methods using this technique are simply referred to as WASEEM and FOUNTA in results Tables~\ref{tab:correlation} and~\ref{tab:performance}.} Rather than using the performance on the source data to estimate target performance, we also evaluate the use of an out-of-domain dataset to quantify the generalization of a model. In this paper, we make use of two third-party out-of-domain datasets: FOUNTA and WASEEM. While both of these datasets are still ``out-of-domain'' when compared to the final test GeoOLID dataset, they still may give practical information about each model's ability to generalize in the context of covariate and label shifts. Formally, to estimate the performance of model $M_i$ on dataset $j$ ($\hat{r}^{\mathcal{M}_i}_j$), we use it's performance on a third party dataset (e.g., FOUNTA) ${r}^{\mathcal{M}_i}_{FOUNTA}$.  It is important to note that both this metric and the source data metric will give the same ranking for every city. 

\vspace{1mm} \noindent \textbf{RV.}
We evaluate the reverse validation variant proposed by \citet{ganin2016domain}. As described in Section~\ref{sec:relwork}, the reverse validation operates in four phases. First, a classifier $\mathcal{M}_i$ is trained on the source dataset. Second, $\mathcal{M}_i$ is applied to the target dataset $j$ and the predictions $\hat{y}_j$ are stored. Third, a new classifier  $\hat{\mathcal{M}}_i$ parameters in the same way as $\mathcal{M}_i$ is trained on the target dataset using $\hat{y}_j$ as the pseudo-labels. Fourth, $\hat{\mathcal{M}}_i$ is applied to the source's development dataset and the resulting performance is used to estimate the target performance ($\hat{r}^{\mathcal{M}_i}_j$). Intuitively, if the predictions $\hat{y}_j$ are accurate, then the resulting models should perform well on the source data.

\vspace{1mm} \noindent \textbf{IWV.}
Another method used for domain adaptation accuracy estimation is Importance Weighted Cross Validation by \citet{sugiyama2007covariate}. We follow a slight variant of the IWV methodology describe in \citet{pmlr-v97-you19a}. IWV has has a three step procedure. Like reverse validation, the first step is to train a model  $\mathcal{M}_i$ on the source data. Second, we train a binary logistic regression classifier $P(c| \mathbf{x})$ on the mid-level features generated from the chosen neural network architecture to predict whether a given instance is from the source or target dataset. Third, we use the source vs. target classifier to weight the evaluation metric performance of $\mathcal{M}_i$  calculated on the source data's validation dataset.

Formally, we define the IWV as
\begin{equation*}
    \hat{r}^{M_i}_j = \frac{1}{D} \sum_{k=1}^{D} w_k\, \mathbb{1}[y_k = \hat{y}_k]
    \label{weighted_acc}
\end{equation*}
where $D$ is the number of examples in the source data's validation dataset, $\mathbb{1}[y_k = \hat{y}_k]$ is a indicator function that tests whether the class $\hat{y}_k$ predicted by $\mathcal{M}_i$  is equal to the ground-truth class $y_k$, and
\begin{equation*}
    w_i = \frac{P(c = j | \mathbf{x}_k)}{P(c = s | \mathbf{x}_k)},
    \label{w_i}
\end{equation*}
where $j$ represents dataset $j$ (the target dataset), $\mathbf{x}_i$ represents the mid-level neural features for example $k$,and $s$ represents the source dataset.
Likewise, $P(c = j | \mathbf{x}_i)$ represents the probability of $\mathbf{x}_i$ (an example from the source validation dataset) being from the target dataset. Similarly, $P(c = s | \mathbf{x}_i)$is the probability of $\mathbf{x}_i$ being from the source dataset. The probabilities are generated from the domain classifier. Intuitively, we are calculating a weighted accuracy on the source validation dataset, where the weights are high for examples in the validation dataset that are similar to target data, and weights are low for examples that are not similar to examples in the target data. 

We also investigate and implement two variances of IWV: IWV and IWV Converse. The only difference between the original and the converse the indicator function is changed from $\mathbb{1}[y_k = \hat{y}_k]$ to $\mathbb{1}[y_k \neq \hat{y}_k]$---weighting incorrect predictions instead of correct predictions.

\vspace{1mm} \noindent \textbf{DEV.}
\citet{pmlr-v97-you19a} also introduced deep embedded validation (DEV). Like the IWV technique, a classifier $P(c | \mathbf{x}_i)$ is trained to predict whether a given example is from the source or target dataset using the mid-level neural represents~$\mathbf{x}_i$.

Basically, DEV differs from IWV in terms of the weighting and performance estimation. Specifically, the weights are defined as
\begin{equation*}
    w_{i} = \frac{D_s}{D_j}\,  \frac{P(c = j | \mathbf{x}_k)}{P(c = s | \mathbf{x}_k)},
    \label{dev_weight}
\end{equation*}
where $D_s$ and $D_j$ represent the number of examples in the source dataset and target datasets, respectively. Next, the performance estimate is calculated as 
\begin{equation*}
    \hat{r}_j^{M_i} = \Big[\sum_{i=1}^D w_i\, \mathbb{1}[y_k = \hat{y}_k]\Big] + \Big[\frac{\eta}{D} \sum_{i=1}^{D} w_i\Big] - \eta
    \label{risk}
\end{equation*}
where
\begin{equation*}
    \eta = - \frac{{cov}(L, W)}{{var}(W)},
\end{equation*}
such that $W = [w_1, \ldots, w_D]$, $L = \big[w_1\, \mathbb{1}[y_1 = \hat{y}_1], \ldots, w_D\, \mathbb{1}[y_D = \hat{y}_D]\big]$, ${cov}(L, W)$ represents the covariance between $L$ and $W$, and ${var}(W)$ represents the variance of $W$. Theoretically, DEV transforms IWV such that it produces an unbiased estimation of the target performance with bounded variance. We refer the reader to \citet{pmlr-v97-you19a}  for more information.

Finally, similar to IWV, we investigate two variances of the DEV model: DEV and DEV Converse. The only difference between the original and the converse version is that the indicator function is changed from $\mathbb{1}[y_k = \hat{y}_k]$ to $\mathbb{1}[y_k \neq \hat{y}_k]$.



\begin{table*}[t]
\setlength\extrarowheight{1pt}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrrrrrrrrrrrr} \toprule
 & \multicolumn{1}{l}{\textbf{Chi}} & \multicolumn{1}{l}{\textbf{Det}} & \multicolumn{1}{l}{\textbf{Bal}} & \multicolumn{1}{l}{\textbf{ElP}} & \multicolumn{1}{l}{\textbf{LA}} & \multicolumn{1}{l}{\textbf{Hou}} & \multicolumn{1}{l}{\textbf{Col}} & \multicolumn{1}{l}{\textbf{Ind}} & \multicolumn{1}{l}{\textbf{Mia}} & \multicolumn{1}{l}{\textbf{Mem}} & \multicolumn{1}{l}{\textbf{NYC}} & \multicolumn{1}{l}{\textbf{NO}} & \multicolumn{1}{l}{\textbf{SA}} & \multicolumn{1}{l}{\textbf{Phi}} & \multicolumn{1}{l}{\textbf{Pho}} & \multicolumn{1}{l}{\textbf{Avg}}  \\ \midrule \midrule
 \multicolumn{16}{c}{\textbf{Baseline}} \\ \midrule
\textbf{Source} & .410 & .380 & .430 & .298 & .223 & .072 & .276 & .359 & .456 & .283 & .349 & .613 & .448 & .405 & -.022 & .332 \\ \midrule \midrule
 \multicolumn{16}{c}{\textbf{Unsupervised Model Selection}} \\ \midrule
\textbf{RV} & {.496} & {.234} & .495 & {.363} & .369 &{.282} & {.267} & .416 & {.194} & .312 & 0{.348} & {.584} &{.525} & {.417} & {.130} & {.362}  \\
\textbf{IWV Conv} & .439 & .352 & .536 & .299 & .271 & .055 & .274 & {.431} &{.493} & .315 & .442 & {.509} & {.393} &{.499} & .000 & .354  \\
\textbf{IWV} & {-.125} & .029 & {-.166} & .011 & .213 & .115 & .193 & {-.049} & {-.028} & {-.111} & {-.121} & {-.043} & {-.005} & {-.218} & {.161} & {-.010} \\
\textbf{DEV Conv} & .415 & {.252} & .542 & .349 & .321 & .193 & {.408} & .370 & {.398} & {.342} & .365 & {.550} & .481 & {.396} &{.179} & .371  \\
\textbf{DEV} & {.391} & {.375} &{.599} & {.167} & {.399} & .126 & .346 & {.431} & {.399} & .293 & {.442} & {.602} & .489 & .405 & .037 & .367 \\ \midrule
%\textbf{PAD} & .000 & .000 & .000 & .000 & .000 & .000 & .000 & .000 & .000 & .000 & .000 & .000 & .000 & .000 & .000 & .000 \\ \midrule
\textbf{Ensemble 1} &{.526} &{.419} & {.569} &{.412} &{.408} & {.268} &{.419} &{.465} & {.447} &{.348} &{.470} &{.673} & {.518} & {.393} & {.145} &{.432}  \\ 
 \midrule \midrule
 \multicolumn{16}{c}{\textbf{Out-of-domain Data for Model Selection}}\\  \midrule
\textbf{WASEEM} & .459 & .360 & .469 & .267 & .488 & .392 & .441 & .475 & .398 & .309 & .399 & .358 & .315 & .571 & .376 & .405 \\
\textbf{FOUNTA} & .562 & .495 & .590 & .542 & .375 & .252 & .444 & .454 & .623 & .510 & .478 & .673 & .616 & .499 & .087 & .480 \\ \midrule
\textbf{Ensemble 2}          & .647 & .516 & .585 & .474 & .491 & .363 & .479 & .502 & .627 & .491 & .515 & .595 & .550 & .720 & .328 & .525    \\ \bottomrule
\end{tabular}%
}
\caption{The Spearman's Rank-Order Correlation results for the 15 cities.\vspace{-1em}}
\label{tab:correlation}
\end{table*}



\vspace{1mm} \noindent \textbf{Ensemble.}
We experiment with three different ensemble methods. First (Ensemble 1), we evaluate an average of the RV, IWV, and DEV metrics, along with IWV and DEV converse forms. Intuitively, this ensemble (and associated parts) can be assume there are no out-of-domain datasets available to test the model. Moreover, they can produce city-specific model rankings, allowing for fine-grained model selection. Second (Ensemble 2), we evaluate an average of the ground-truth on the two ``Third-Party Out-of-Domain Datasets'': FOUNTA and WASEEM. This ensemble and associated parts evaulate the performance of ranking all cities in the same way based on how the models generalize on a third-party dataset. %Third, we evaluate a simple weighted combination of FOUNTA+Ensemble 1 and WASEEM+Ensemble 1, where the performance scores are calculated as $\alpha\, \mathbf{e}_1 + (1-\alpha)\, \mathbf{e}_2$ such that $\alpha \in [0, 1]$ and $\mathbf{e}_b$ represents the performances estiamtes for both FOUNTA/WASEEM and Ensemble 1, respectively. $\alpha$ is chosen by its performance on a the held-out dataset (e,g., WASEEM for FOUNTA+Ensemble 1).



%This allows us to run any experiment we want on unlabeled data and estimate how it performs once deployed. With multiple models trained and kept during the iterative model building process, we can grab sub-samples of the data they are expected to receive once deployed. We can used the trained ensemble model to estimate the accuracy of every model/embedding pair and deploy the best model in various situations.
\end{comment}

==> Sections/OLD_TaskDefinition.tex <==
\begin{comment}
\begin{figure*}
\centering
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=\linewidth]{correlation.pdf}
    \caption{Spearman rho correlation between the ground-truth ranked performance between two cities.}
    \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=\linewidth]{correlation2.pdf}
    \caption{Spearman rho correlation between the ensemble-based ranked performance estimates between two cities.}
  \label{fig:sub2}
\end{subfigure}
\caption{A figure with two subfigures}
\label{fig:test}
\end{figure*}
\end{comment}

\begin{comment}
The goal of this paper is to find methods that can effectively rank the performance of diverse methods on out-of-domain data. Formally, let $\mathcal{M}_i$ represent a model trained on dataset $i$, $r^{\mathcal{M}_{i}}_j$ represents the ground truth performance metric (e.g., Accuracy) resulting from applying model $\mathcal{M}_i$ to dataset $j$, and $\hat{r}^{\mathcal{M}_{i}}_{j}$ is the estimated performance metric. The task defined in this paper is to evaluate the correlation between $\mathbf{r}_j= [r^{\mathcal{M}_{i}}_1, \ldots, r^{\mathcal{M}_{N}}_j]$ and $\mathbf{\hat{r}}_j = [\hat{r}^{\mathcal{M}_{i}}_1, \ldots, \hat{r}^{\mathcal{M}_{N}}_{j}]$, where $N$ is the total number of models. Moreover, we evaluate using traditional metric used in unsupervised domain adaptation model selection literature. Specifically, let $u_e = \argmax_i \hat{r}^{\mathcal{M}_{i}}_j$ represent the index of the model with the highest estimate performance (e.g., with reverse validation) on dataset $j$. Likewise, let $u_s = \argmax_i s^{\mathcal{M}_{i}}_j$ represent the best predicted model using the model $M_i$'s performance on the source data $s$ as an estimate of target performance. The goal for the traditional of the model ranking task is for the best model detected by the model selection metric $r^{\mathcal{M}_{u_e}}_j$ to be better then the best model chosen using the model's performance on the source data as a estimate of target performance ($r^{\mathcal{M}_{u_s}}_j$). Intuitively, a metric that both maximizes correlation and performance is more robust (i.e., better) than a metric that only performs well on one. But, again it is important to note that the second metric does not incorporate information about the relative ranking of all tested models. To the best of our knowledge, this is the first paper to the ranking correlation of model selection methods.

The first part of training consisted of training the deep learning models on a source dataset and then testing on a target dataset. In the training phase of the offensive language classifiers, all 3 datasets (FOUNTA, WASEEM, OLID) are used throughout NLP research and provide widely accepted labels for the task. This allowed us to train multiple models on predicting the same task, simulating the iterative process of model building, and get the true accuracy on how it performs on the target dataset. This was done for every combination of the three datasets. 

With all the models trained for offensive language and kept, instead of thrown away, we apply the multiple out of domain performance techniques mentioned in the Methods section. This creates features for our ensemble model to use to predict the true accuracy on how it will perform on out of domain data. The ensemble model uses the outputs from Reverse Validation, Importance Weighted, Deep Embedding, 	Deep Embedding Converse to predict the true out of domain performance obtained by the direct method. 

What training this ensemble did was gave us a technique to predict the performance via true accuracy of a model and a dataset that is not labeled for the task at hand. By saving all the trained models implemented during the iterative model building step of machine learning, we can rank all models against different target datasets and deploy the one with the highest estimated accuracy.

With our ensemble model trained and fine-tuned on the 3 datasets, we want to validate our model and test it against data that it would see in a deployed setting. We test our model and methods on the Geo Offensive Language Identification Dataset which allows us to validate our model against 15 geographically and demographically diverse cities for offensive language detection. The same steps mentioned above are followed to obtain the true accuracy of dataset so the performance of the ensemble model can be measured. Every models performance is evaluated with the ensemble model and then ranked by highest estimated performance. The model with the highest ranking is chosen as the best model to deploy. This is done for all 15 cities and the results of the experiments are discussed in the next section. 
\end{comment}

%%% Implement PAD* and why we chose to use it
%%% NLPERF Argue why it doesnt fit the scope of our research



==> Sections/RelatedWork.tex <==
\section{Language Variation}

Langauge variation is an important area of research for the NLP community. For example, understanding how different languages vary (e.g., Finnish vs Korean) typologically has been shown to be important to reduce performance disparities of language models~\cite{gerz2018relation}. While there has been some disagreement about whether morphology matters, recent work by \cite{park2021morphology} has shown that incorporating information that can model morphological differences is important in improving model performance. Overall, much of the prior work has focused on either developing methods to identify language features within text or use various language features to improve model performance. For instance, VarDial Evaluation has been an annual competition to identify various dialects of different languages (e.g., German and Romanian) as well as geolocations~\cite{gaman2020report}.
%One of the shared tasks present was Social Media Variety Geolocation (SMG), where teams competed to construct a classifier that could predict the coordinate points of a piece of text with high accuracy \cite{gaman2020report}.
For instance, \citet{cheke2020understanding} use topic distributions to show that different topics can provide signal to determine where the text originated from. For the same shared task, \citet{scherrer2021social} show that combining modern NLP architectures like BERT with a double regression model can also provide success in determining the latitude and logitude points of the location of the text. The results of this shared task highlights the fact that semantic and lexical differences exist when locations of the text change. Other work around regional variation of language \cite{hovy2018capturing, hovy2020visualizing, kellert2021geolocation} further prove that these differences in dialect and lexical patterns are significant across geographies.

% , especially work comparing language variation with geographic information,
 Overall, the major gap in prior work looking and language variation is that there has not been any studies evaluating the impact regional language variation has on the performance of downstream tasks. In this paper, we introduce a novel dataset called GeoOLID. However, before addressing the research gap in understanding performance disparities, it is important to measure language variation across each city within the dataset. If cities do not vary with regards to content and langauge style, then we should not expect models to perform different within each city. Hence, we test the following hypothesis:
\begin{itemize}[wide =0pt, labelwidth=\widthof{H1a.},topsep=5pt]%[start=1,label={\bfseries H\arabic*):},align=left,widest=ii, labelsep=0pt,leftmargin=*]
\itemsep-.5em 
\item[\textbf{H1a.}] Text in the GeoOLID dataset is distributed differently (based on content and style) depending on the location it was posted. 
\item[\textbf{H1b.}] Text is representative of the sociodemographic makeup of the area it was posted.
\end{itemize}
By expanding the analysis of prior work looking at dialectal variation~ \cite{abdul2020toward, lulu2018automatic, blodgett2016demographic}, we are able show that the results generalize to our newly collected dataset.
%Specifically, we .
%By combining the 2 fields of research along with prior work in dialect and location prediction \cite{abdul2020toward, lulu2018automatic, blodgett2016demographic}, we fill a hole in research by measuring the performance of task classification across difference geographies.


\section{Performance Disparities}

%\textcolor{blue}{While there is a gap in current research around measuring and analyzing geographic performance of NLP classifiers, researchers have investigated performance and geographic disparities. There has a plethora of research done in discovering disparities in the models performance across different languages and dialects. In addition to that branch of research, there has been research published that measures geographic disparities that arise in textual data.}

Performance disparities across languages and dialects recently have seen received much attention in NLP. For example, recent research shows that performance drops in text classification models across different sub-populations such as gender, race, and minority dialects \cite{dixon2018measuring, park2018reducing, badjatiya2019stereotypical, rios2020fuzze, lwowski2021risk, mozafari2020hate}. \citet{sap2019risk} measure the bias of offensive language detection models on AAE. Likewise, \citet{park2018reducing} measure gender bias of abusive language detection models and evaluate various methods such as word embedding debiasing and data augmentation to improve biased methods.  \citet{davidson2019racial} shows that there is racial and ethnic bias when identifying hate speech online and show that tweets in the black-aligned corpus are more likely to get assigned as hate speech. Overall, performance disparities have been observed across a wide array of NLP tasks such as detecting virus-related text~\cite{lwowski2021risk}, coreference resolution~\cite{zhao2018gender}, named entity recognition~\cite{mehrabi2020man}, and machine translation~\cite{font2019equalizing}.

%These performance issues is what naturally peaked our interest in testing H2 and H3, that model performance can vary due to the distribution of the data differing between locations and is the best model the same for every city.

Overall, the major research gap in prior work is in the lack of fine-grained regional understanding of performance disparities. Many groups that are studied are broad, such as male vs. female (using an unrealistic assumption of binary gender~\cite{rios2020quantifying}), or AAE which is not universally spoken in the same way within different cities in the US. For example, \citet{jones2015toward} show that many well-known AAE patterns (e.g., sholl, an nonstandard spelling of ``sure'') do not appear uniformly across the US. Hence, if an Offensive language detection model performs poorly on one set of AAE patterns, it can impact one region much  more than others. Unfortunately, it is neither possible to measure model performance for every minority sub-population nor all potential syntactic pattern given the ever evolving nature of language. Furthermore, it is not possible to understand how a model will perform on every ``common'' topic discussed within the US given the large variation in discussions (e.g., Texas may speak more about the Dallas Cowboys, while Ohio focuses on the Bengals for the topic of Football). Hence, we believe that community-driven analysis is a better future avenue to understand the real-world impact of NLP models. Instead of trying to understand all potential sub-populations and style variations to evaluate them all, we propose measuring performance on small communities instead. Overall, to begin addressing these gaps in understanding, we make the following hypothesis:
\begin{itemize}[wide =0pt, labelwidth=\widthof{H1a.},topsep=5pt]%[start=1,label={\bfseries H\arabic*):},align=left,widest=ii, labelsep=0pt,leftmargin=*]
\itemsep-.5em 
\item[\textbf{H2a.}] Because data is distributed differently in different geographic regions, model performance is not the same in each location.
\item[\textbf{H2b.}] Errors made by the models are caused by geographic-specific content and language style.
\item[\textbf{H3.}] Model choice depends on the community it will be deployed.
\end{itemize}
These hypotheses will provide a starting point towards what we term ``community-driven NLP''. By showing that model performance can vary location-to-location, we hope to bring awareness of adverse harms that the broad application of NLP can cause without carefully understanding the communities in which the models are deployed.



































\begin{comment}
In this section, we describe two main research areas related to this work: Unsupervised (Unsup) Domain Adaptation Model Selection and Predictive Performance.


\vspace{1mm} \noindent \textbf{Unsup. Domain Adaptation Model Selection.}
Machine learning models struggle to generalize as data changes over time or the general data distribution between the source dataset and target dataset changes. A wide range of methods developed to detect shifts in the data distribution and predict data shift's impact on model performance. For instance, \citet{Hsu_2020_CVPR}, \citet{van-asch-daelemans-2010-using}, and \citet{lee2018simple} proposed methods of detecting specific out-of-domain examples. \citet{techapanurak2021practical} provided a comprehensive review of out-of-domain detection methods. \citet{kashyap2020domain} explore multiple metrics to measure domain divergence and evaluate their role in estimating a model's out-of-domain performance. Similarly, \citet{elsahar2019annotate} evaluate three different methods for predicting the performance drop on data that is not annotated. However, contrary to our work, their work looked at predicting a performance drop will happen, not necessarily exploring the magnitude of the drop nor its relationship to other models. In contrast, this paper explores methods of ranking the relative performance of different models. 


Several researchers have developed unsupervised domain adaptation model selection methods. \citet{sugiyama2007covariate} introduced importance-weighted cross-validation, which provides example-wise weighting of the performance metrics calculated using the source data's validation set to estimate target performing. The weighting uses a density ratio of the probability of an example being in the source vs. target dataset. \citet{pmlr-v97-you19a} improved upon the importance-weighted validation procedure to improve its application to neural network-based models. Transfer cross-validation is another approach used to estimate unlabeled out-of-domain target data~\cite{zhong2010cross,ganin2016domain}. For the \citet{ganin2016domain} variant, for a set of hyperparameters, the reverse validation ``performance'' can be estimated by first splitting source (labeled) and target (unlabeled) data into training and validation sets. Then, the labeled source and unlabeled target data are used to learn a classifier (as is usually done). Next, this classifier is used to label the target data, and a new ``reverse'' classifier is learned (with the same algorithm) using the pseudo-labeled target data (as as a synthetic ``source``) and the unlabeled source data (as fake ``target'', i.e., ignoring the known labels). This reverse classifier is evaluated on the source validation data to estimate the target performance. This paper extends prior studies in two ways. First, prior work has looked at the performance increase using a new metric over other similar metrics or simply overusing the best model evaluated on the source data. The \textit{gap} in prior literature is how well these metrics rank the models between one another. It is unknown whether the metrics provide fine-grained information to compare models. Second, prior work has only used the metrics to choose hyperparameters. This paper explore how they generalize when comparing different~architectures.

\vspace{1mm} \noindent \textbf{Predictive Performance.}
Another recent trend that is related to this paper is in the area of predictive performance~\cite{ye2021towards,xia2020predicting}. \citet{xia2020predicting} introduces a regression model based on various features (e.g., number of words in common between two datasets and a categorical for model type) to predict the performance. Similarly, \citet{ye2021towards} expand on the work by \citet{xia2020predicting} for more fine-grained performance prediction with domain divergence for NLP. Specifically, they introduce data partitions and a novel tensor-decomposition method to answer questions such as ``what are the accuracies for entity recognition by entity length?'' Overall, prior predictive performance methods differ from this paper in two ways. First, they are fundamentally about predicting performance \textit{before} the model is trained. Thus, they use a general categorical (one-hot encoded) feature representing a model. In contrast, we are interested in fine-grained relationships between both slight variants of a model (e.g., a model trained with a learning rate of 1e-3 vs. 1e-6). Second, their evaluation strategy focused on minimizing the root mean squared error (RMSE) between the predicted and actual performances. Nevertheless, the \textit{gap} missing in terms of evaluation is how the models are ranked between one another. A small RMSE score does not necessarily mean models will be ranked correctly, especially if performance differences are small between two models.


%The first method is based $\mathcal{H}$-divergence based metrics. They use a variation Proxy $\mathcal{A}$-Distance(PAD) they call \textbf{PAD*}. Given 2 datasets $D_{s}$(source) and $D_{t}$(target), a neural network classifier is trained on the source dataset and the authors want to estimate the accuracy on the target. This is accomplished by passing samples form both the $D_{s}$ and $D_{t}$ through the network and capturing the hidden representation of the last layer for each sample. With each input being transformed into its hidden representation, a linear model is then trained to predict if an example comes from source or the target dataset. In the methods and experiments section we implement PAD* to compare our ensemble model to their method. that predicts the accuracy of a model $\mathcal{M}$ for a task $\mathcal{T}$ trained on dataset $\mathcal{D}$ on a test dataset $\mathcal{D^{\prime}}$. For their experiments they choose a gradient boosted tree model that take different dataset level features as its inputs and the true accuracy of the metric as the outputs. Some examples of the dataset level features includes the size of the dataset, vocabulary size, average sentence length, and word overlap. Although this method is useful, we do not implement it on our study due to our problem and approach being different. They use a categorical variable for each model tested in order to select the best model. In our case we test 3 different models, over 20 different word embeddings. This would create a large sparse input vector into our ensemble model which we try to avoid. 

\end{comment}

==> Sections/Results.tex <==


\begin{comment}


\begin{table*}[t]
\setlength\extrarowheight{1pt}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lllllllllllllllll@{}}
\toprule
 & \textbf{Chi} & \textbf{Det} & \textbf{Bal} & \textbf{ELP} & \textbf{LA} & \textbf{Hou} & \textbf{Col} & \textbf{Ind} & \textbf{Mia} & \textbf{Mem} & \textbf{NYC} & \textbf{NO} & \textbf{SA} & \textbf{Phi} & \textbf{Pho} & \textbf{AVG} \\ \midrule \midrule
 \multicolumn{16}{c}{\textbf{Baseline}} \\ \midrule
\textbf{Source}        & .785 & .748 & .779 & .739 & .771 & .733 & .750 & .757 & .806 & .739 & .803 & .787 & .758 & .771 & .694 & .761 \\ \midrule \midrule
 \multicolumn{16}{c}{\textbf{Unsupervised Model Selection}} \\ \midrule
\textbf{RV}   & {.822} & {.781} & .810 & {.786} & {.797} & {.759} & {.785} & {.741} & {.860} & {.739} & {.818} & {.805} & {.795} & .789 & {.727} & {.788} \\
\textbf{IWV}     & {.809} & .758 & {.812} & {.764} & .773 & {.732} & {.782} & {.789} & {.855} & .750 & {.817} & {.759} & {.752} & .789 & {.724} & .778 \\
\textbf{IWV Conv}           & .809 & .758 & .812 & .764 & .773 & .732 & .782 & .789 & .855 & .750 & .817 & .759 & .752 & .789 & .724 & .778 \\ 
\textbf{DEV}     & {.809} & .758 & {.812} & .746 & {.807} & {.763} & .776 & {.782} & {.855} & {.775} & {.817} & .801 & {.752} & .790 & {.724} & .785 \\
\textbf{DEV Conv} & {.809} & .758 & {.813} & .746 & {.807} & {.763} & .776 & {.782} & {.855} & .774 & {.817} & .801 & {.752} & {.799} & {.724} & .785 \\ \midrule
%\textbf{PAD}           &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      \\ \midrule 
\textbf{Ensemble 1}      & {.809} & {.781} & .805 & .749 & {.807} & {.759} & {.785} & {.782} & {.855} & {.780} & {.799} & {.811} & {.784} & {.798} & {.724} & {.789} \\  \midrule  \midrule
 \multicolumn{16}{c}{\textbf{Out-of-domain Data for Model Selection}}\\  \midrule
\textbf{WASEEM} & .807 & .761 & .813 & .766 & .786 & .755 & .776 & .782 & .853 & .774 & .818 & .799 & .774 & .799 & .720 & .786 \\
\textbf{FOUNTA} & .822 & .781 & .810 & .786 & .797 & .767 & .795 & .784 & .860 & .781 & .818 & .825 & .795 & .789 & .739 & .797 \\ \midrule
\textbf{Ensemble 2}        & .807 & .761 & .813 & .766 & .786 & .755 & .776 & .782 & .853 & .774 & .818 & .799 & .774 & .799 & .720 & .786  \\ \bottomrule
\end{tabular}%
}
\caption{Overall Performance (Accuracy) when selecting the best model based on each of the out of domain performance estimation.\vspace{-1em}}
\label{tab:performance}
\end{table*}


\vspace{1mm} \noindent \textbf{Spearman's Rho Correlation Experiments.}
We first evaluate the correlation between the estimated performance rankings $\hat{\mathbf{r}}$ for each method with the ground-truth model rankings $\mathbf{r}$. The results are listed in Table~\ref{tab:correlation}. First, for the Unsupervised Model Selection methods, we find that no single approach is robust across all datasets. While all methods except for the standard IWV method outperform rankings based on Source performance, a simple average (Ensemble 1) produces the best results with an Avg correlation of .432, compared the the next best DEV Conv with a score of .371. Moreover, we find that the average method does not substantially perform worse than the Source rankings, while all other metrics perform substantial worse in terms of correlation for at least one city. Finally, we also find that the rankings can vary substantially across all metrics. For instance, the correlation using the source dataset for Houston (Hou) is only .072. Yet, highest correlation using the source ranking is for New Orleans (NO) with a Spearman's rho score of .613. Interestingly, this indicates substantial variation across cities with regards to best model selection. Based on these results, it is unreasonable to assume a single method will generalize at the scale of many internet companies, even when the scale is limited to English tweets within the continental US.

Second, for the experiments in which we use the performance third-party out-of-domain dataset to rank the models for each city, we find both metrics perform nearly as good or better than Ensemble 1. Specifically, ranking the models based on their performance on the WASEEM dataset achieves and average correlation of .405. Likewise, the ranking models based on their performance on FOUNTA achieves an average correlation of .48. The Ensemble (average) of the WASEEM and FOUNTA model performance scores (Ensemble 2) results in an average ranking of .525. Overall, these findings are interesting because they suggest that the \textit{broad} generalization performance of certain models in the presence of covariate, label, and potentially concept shift is more important than fine-grained differences across cities. In the context of offensive language detection, their have been many curated datasets, thus using a slightly different dataset to estimate generalization at large may be a good solution rather using the Unsupervised Domain Adaptation Model Selection Methods. However, when such out-of-domain datasets do not exist, using an Ensemble of multiple Unsupervised Domain Adaptation Model Selection Methods is suggested. Furthermore, when multiple out-of-domain datasets exist, averaging performance metrics for each model is an easy way to improve model choice selection.


%Each method mentioned implemented had all variations of model and word embeddings ranked from best model to worst model. The direct method gave us the true rankings on how the model/word embedding pair performed on the target city dataset. The Spearman's Rank-Order Correlation provides us a way to measure the correlation between the two ranked lists. If the correlation is close to 1 then the method does a perfect job of finding the best classifier to deploy. The results of all methods and the correlations to the true performance are provided in table

%Some major takeaways from the results is first, our ensemble model obtains the highest correlation score compared to all other methods on 9 out of the 15 cities and top 2 on 13 of the 15.. This shows that when using our trained ensemble model selection technique, we will be more likely to deploy the best model in a more personalized manor versus the other techniques. This allows model builders to deploy more personalized models across different sub groups while maintaining high performance.

%Another takeaway is to take average correlation across the methods to show how well it generalized. Once again the ensemble model obtains the highest correlation compared to the other methods.





\vspace{1mm} \noindent \textbf{Performance Increase Experiments.}
In Table~\ref{tab:performance}, we report the results (Accuracy) of choosing the best model based on each estimate of the target datasets performance. Overall, compared to the correlation results, every method results in similar performance gains. Moreover, on average, all methods result in better performance than simply using the Source dataset to estimate out-of-domain performance. For instance, the average Accuracy is .785 using both the DEV Conv Method and .786 using the WASEEM approach, even though the there were substantial differences in correlation. The results imply that prior evaluation methodologies for model selection metrics do not provide a comprehensive view about a certain metrics performance. For instance, a metric may get luck a few times, reporting the best model simply by chance. Thus, it is our recommendation that rank-based metrics (e.g., Spearman's rho) be used to help differentiate the quality of future metrics proposed by researchers.

%Not only is there a high correlation between our ensemble model and the actual accuracy of the classifier, but by using the rankings from the model to choose the best model to deploy provides lift to the overall performance. We see a 1-3\% accuracy increase when choosing the best model based on the ensemble model vs all other methods including the source. We see that in table \ref{tab:performance} that the ensemble model achieves the highest accuracy in 8 out of the 15 cities as well as the average performance across all cities. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{correlation.pdf}
    \caption{Spearman rho correlation between the ground-truth ranked performance between two cities.\vspace{-1em}}
    \label{fig:cross}
\end{figure}

\vspace{1mm} \noindent \textbf{Cross-Dataset Correlation.}
In Figure~\ref{fig:cross}, we report Spearman's rho correlation between the ground-truth $\mathbf{r}_j$ for each pair of datasets. For instance, the Figure provides insight that the correlation between the ground-truth rankings of New Orleans and Phoenix is below .6. This finding is substantial because it suggests that if you can annotate data similar to your target dataset, then you can beat the performance of using highly out-of-domain data as well as the performance of Unsupervised Domain Adaptation Model Selection Methods (in this case we can assume Phoenix and New Orleans are similar, but differ only slightly in terms of small ``shifts''). However, there is still substantial variation in terms of correlations, ranging from .5 to nearly .9. Thus, this suggests there is substantial room for improvement that current approaches for out-of-domain model selection---nor simple combinations of existing approaches---do not solve. We hope this dataset facilitates future work in the development of novel unsupervised domain adaptation model selection metrics.
\end{comment}

\begin{comment}
\vspace{1mm} \noindent \textbf{Implications.}

{it is better to use a combination}

{other implication}.

{measuring the quality of unsupervised domain adaptation model selection methods by measuring the best chosen models performance is not adequate by itself}.
\end{comment}
